DUET: Agentic Design Understanding via Experimentation and Testing

AI agents powered by large language models (LLMs) are being used to solve increasingly complex software engineering challenges, but struggle with hardware design tasks. Register Transfer Level (RTL) code presents a unique challenge for LLMs, as it encodes complex, dynamic, time-evolving behaviors using the low-level language features of SystemVerilog. LLMs struggle to infer these complex behaviors from the syntax of RTL alone, which limits their ability to complete all downstream tasks like code completion, documentation, or verification. In response to this issue, we present DUET: a general methodology for developing Design Understanding via Experimentation and Testing. DUET mimics how hardware design experts develop an understanding of complex designs: not just via a one-off readthrough of the RTL, but via iterative experimentation using a number of tools. DUET iteratively generates hypotheses, tests them with EDA tools (e.g., simulation, waveform inspection, and formal verification), and integrates the results to build a bottom-up understanding of the design. In our evaluations, we show that DUET improves AI agent performance on formal verification, when compared to a baseline flow without experimentation.

==> text/evaluation-from-abstract.tex <==
\section{Case Study and Summary of Results}
\label{sec:eval}

% In evaluating \sys{}, 
%   the primary research question
%   we seek to answer is,
%   \textbf{does the \sys{} experiment report
%     improve AI agent performance on hardware design tasks?}
% To evaluate this question,
%   we integrate \sys{}
%   into AI hardware verification agents.

% In this section, we describe
%   an example from our evaluation
%   which clearly demonstrates 
%   the positive effects of the
%   \sys{} experiment report.

\paragraph*{Experiment setup}
We build a \textit{black box verification} AI agent,
  which iteratively attempts to verify
  a single feature of a design
  in simulation,
  given only
  natural language
  documents
  describing the design. 
% The agent is then asked 
%   to verify the requested feature
%   of the design
%   by constructing a simulation testbench
%   with ample assertions.
The agent's performance
  on the task 
  gives us a measure of the quality
  of the input documents.
To evaluate \sys{}, we run
  the black box verification agent
  using two sets of inputs,
  in two scenarios we label
  \textsc{Rtl-Only}
  and \sys,
  and compare their outputs.
% We allow the agent to autocorrect
%   compilation errors,
%   failing assertions,
%   and testbench timeouts.
% Crucially, we provide no logs
%   in assertion failure or timeout cases
%   to avoid giving the agent feedback on the RTL.
% We run the black box verification agent
%   and collect statistics on the number of autocorrect iterations,
%   the runtime,
%   and the number of assertions in the produced testbench,
%   among other numbers.
% We also manually check
%   whether the testbench truly verifies the specified feature.
We use Verilator as our simulator.
% Testbench timeout is set to five seconds.
All LLM queries use GPT-5.0.

\paragraph*{Target design and feature}
We target the OpenTitan \iicmod{}
   submodule\footnote{
\url{https://github.com/lowRISC/opentitan/blob/a14e715d0f425bc4986be526bc52bdeb901756bf/hw/ip/i2c/rtl/i2c\_target\_fsm.sv}
  },
  a complex FSM
  at the core of OpenTitan's \iic{} implementation.
% While the module is not overly complex
%   ($\sim$1000 lines of code),
% The module is a perfect example of what we described
%   in \cref{sec:intro}:
%   a module with complex, dynamic behavior
%   which is not readily apparent from reading its RTL.
The feature to be verified is I$^2$C 
  TX-path clock stretching.
% Note that, while OpenTitan is open source and thus likely
%   in GPT-5's training dataset,
%   we will nonetheless see that baseline performance
%   on this design is still subpar.
 

\paragraph*{\baseline{} vs. \textsc{Duet}} 
To evaluate the quality of \sys{}'s output,
  we execute two different scenarios,
  running our verification agent
  with two different sets of inputs.
  \begin{enumerate}
      \item \textbf{\baseline{}}: we use LLM queries
  to generate (1) a specification of the design
  and (2) a detailed description of the clock stretching feature,
  passing the RTL into the LLM as context.
      \item \textbf{\sys{}}: we run the \sys{} \textsc{\doExperiment}
  routine on the feature to produce an experiment report.
We then use an LLM query
  to enhance the \baseline{} 
  specification and feature description
  using the experiment report.
The \sys{} experiment report, \sys{}-enhanced spec, and \sys{}-enhanced feature description
  are used as the inputs in the \sys{} scenario.
  \end{enumerate}
% In the \baseline{} scenario,
%   we use LLM queries
%   to generate (1) a specification of the design
%   and (2) a detailed description of the clock stretching feature,
%   passing the RTL into the LLM as context.
  % we simply use the specification and feature description
  % as the input
  % to the black box verification agent. \chandra{was this really naive? or did we do any prompt tuning here? is it from our current mental model flow? if so, we could probably say that: we use a ``chain of sequential LLM calls carefully designed to do this". I think its important to explain that the baseline is not weak. }
% In the \sys{} case,
%   we run the \sys{} \textsc{\doExperiment}
%   routine on the feature to produce an experiment report.
% We then use an LLM query
%   to enhance the \baseline{} 
%   specification and feature description
%   using the experiment report.
% The \sys{} experiment report, \sys{}-enhanced spec, and \sys{}-enhanced feature description
%   are used as the inputs in the \sys{} scenario.

\paragraph*{Results and analysis}
The results are captured in this table:

\begin{table}[h]
\centering
\begin{tabular}{c|c|c|c|c}
& \textsc{\doExperiment} Runtime &  Verification iters &Verification runtime & Verified feature?  \\
\hline
     \baseline{} &   N/A & 10 &20m59s & no\\
    \textsc{Duet}&   10m40s (5 iters) &2 & 4m44s & yes \\
\end{tabular}
\end{table}

\sys{}
   significantly outperforms the \baseline{} scenario.
The \baseline{} scenario failed to produce
  a working testbench after 10 iterations;
  all failures were due to failing assertions in the testbench.
The \textsc{Duet} scenario produced a working testbench
  on the second attempt; the first attempt
  produced a testbench which timed out after five seconds.
Manual inspection shows that the \textsc{Duet} 
  testbench successfully exercises the TX clock stretching feature,
  and all nine assertions pass.
Below are snippets from the experiment run\footnote{
  In the full paper, we will include full experiment logs.
}:

\input{text/eval-figure}

The first column shows a snippet of the feature description 
  generated by the \baseline{} approach,
  which, as we will see, is missing a key detail.
The second column shows snippets from two iterations
  of the \sys{} experimentation loop.
The first snippet shows a relevant testbench log
  in which the design behaved contrary to
  the agent's expectations.
The second snippet shows a note
  containing the agent's analysis of the failure.
The agent uses the analysis to fix the testbench
  in later iterations, and successfully exercises the feature.
This pair of snippets concisely demonstrates \sys{}'s ability
  to produce deeper design understanding via experimentation.
Finally,
  the last column shows the enhanced
  feature description produced using
  the \sys{} experimentation report;
  this enhanced feature description was key
  to producing a working testbench
  in the \textsc{Duet} scenario.



==> text/first-page-figure-v1.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=1\textwidth]{assets/DUET.drawio.png}
    
    \caption{
\textbf{Top}: An RTL-only AI agent flow
  executes a hardware design task (``example query'')
  providing only the RTL of the design 
  to the LLM.
\textbf{Bottom}: \sys{} improves on the RTL-only flow
  by introducing an LLM-driven agentic experimentation loop
  which generates a deeper understanding of the design
  and results in higher quality output.
% The resulting experiment 
%   report is then used as additional context
%   when executing the task,
%   leading to higher-quality output.
}
    \label{fig:page1}
\end{figure}

% \begin{tikzpicture}[node distance=1.5cm and 2cm]

% % Top row
% \node[box] (design) {Design};
% \node[box, right=of design] (query) {Query};

% % Naive prompt path
% \node[box, below=1.5cm of design] (naive) {Design \\ (Naïve Prompt)};
% \draw[arrow] (design) -- (naive);
% \draw[arrow] (query) -- (naive);
% \node[box, right=of naive] (response) {Response};

% \draw[arrow] (naive) -- (response);

% % DUET
% % \node[box, below=of query] (duet) {DUET};
% % \draw[arrow] (query) -- (duet);
% % \draw[arrow] (design) -- (duet);

% % Stimulus → EDA → Logs
% % \node[box, below left=2cm and -0.5cm of duet] (stimulus) {Stimulus};
% % \node[box, right=of stimulus] (eda) {EDA};
% \node[box, right=of eda] (logs) {Logs};

% % \draw[arrow] (duet) -- (stimulus);
% % \draw[arrow] (stimulus) -- (eda);
% % \draw[arrow] (eda) -- (logs);

% % New DUET Response
% \node[box, below=2cm of logs] (newduet) {New DUET Response};
% % \draw[arrow] (logs) -- (newduet);

% \end{tikzpicture}
